Uncertainty Quantification and Experimental Design for Large-Scale Linear Inverse Problems under Gaussian Process Priors

We consider the use of Gaussian process (GP) priors for solving inverse problems in a Bayesian framework. As is well known, the computational complexity of GPs scales cubically in the number of datapoints. We here show that in the context of inverse problems involving integral operators, one faces additional difficulties that hinder inversion on large grids. Furthermore, in that context, covariance matrices can become too large to be stored. By leveraging results about sequential disintegrations of Gaussian measures, we are able to introduce an implicit representation of posterior covariance matrices that reduces the memory footprint by only storing low rank intermediate matrices, while allowing individual elements to be accessed on-the-fly without needing to build full posterior covariance matrices. Moreover, it allows for fast sequential inclusion of new observations. These features are crucial when considering sequential experimental design tasks. We demonstrate our approach by computing sequential data collection plans for excursion set recovery for a gravimetric inverse problem, where the goal is to provide fine resolution estimates of high density regions inside the Stromboli volcano, Italy. Sequential data collection plans are computed by extending the weighted integrated variance reduction (wIVR) criterion to inverse problems. Our results show that this criterion is able to significantly reduce the uncertainty on the excursion volume, reaching close to minimal levels of residual uncertainty. Overall, our techniques allow the advantages of probabilistic models to be brought to bear on large-scale inverse problems arising in the natural sciences.

==> gp_regression.tex <==
\section{Infinite Dimensional Inversion: Conditioning Gaussian Random Elements in Banach Spaces}\label{sec:infinite_dim_formulation}
When treating inverse problems with a Bayesian framework, one needs to define priors over spaces of functions. We will restrict ourselves to continuous functions defined over a compact subset $D\subset \mathbb{R}^d$ of Euclidean space. Hence, let $C(D)$ denote the Banach space of continuous functions over $D$ endowed with the sup-norm / the topology of uniform convergence. Solving an \textit{inverse problem} then resorts to the task of inverting the relation $G:C(D)\rightarrow \mathbb{R}^{\datdim}$, where $G$ is a bounded linear operator. To achieve this, we define a prior over $C(D)$ and then compute the posterior distribution given data observed under noise.\\
~\\
As a simple example of an inverse problem falling in this setting, we consider the task of learning a continuous function defined on the interval $\left[-1, 1\right]$ via different types of data: pointwise function values, integrals of the function, Fourier coefficients, etc. \cref{fig:fourier_variance_reduction} provides an illustration of solutions obtained under a Gaussian process prior. Note that the Five different combinations of observations in \cref{fig:fourier_variance_reduction} can be described as a linear operator $G:C\left(\left[-1, 1\right]\right)\rightarrow\mathbb{R}^{\datdim}$
\begin{figure}[tbhp]
\centering
\subfloat[prior]{\includegraphics[scale=0.48]{images/1d_example/variance_prior-eps-converted-to.pdf}}
\subfloat[pointwise]{\includegraphics[scale=0.48]{images/1d_example/variance_1-eps-converted-to.pdf}}\\
\subfloat[pointwise + integral]{\includegraphics[scale=0.48]{images/1d_example/variance_2-eps-converted-to.pdf}}
\subfloat[pointwise + integral + Fourier]{\includegraphics[scale=0.48]{images/1d_example/variance_4-eps-converted-to.pdf}}
\caption{Conditional mean (blue) and 2$\sigma$ credible interval after inclusion of different types of data: (a) prior samples, (b) pointwise data at 3 locations, (c) pointwise data + integral over domain, (d) pointwise data + integral over domain + first two Fourier coefficients. The true unknown function is shown in dashed black.
}
\label{fig:fourier_variance_reduction}
\end{figure}

Gaussian processes provide a convenient class of priors on function spaces and are particularly useful as priors in Bayesian inverse problems. Nevertheless, for theoretical inquiries, the equivalent language of Gaussian measures and disintegrations is often preferred. This frameworks provides several advantages, such as enabling one to formulate discretization-independent algorithms \citep{stuart_cotter} and it also makes clear which types of observations are allowed (namely only elements of the dual space). In \cref{sec:process_measure_equivalence}, we provide theoretical background and show the equivalence between the Gaussian Process and the Gaussian measure formulation of Bayesian inverse problems. In \cref{sec:disintegration}, we derive the posterior in the Gaussian measure formulation by extending results from \citet{TARIELADZE2007851} and make the link to the usual conditioning formulae as found four example in \citet{tarantola}. Finally, we will consider sequential data assimilation problems and prove our main \textit{sequential conditioning theorem} in \cref{sec:sequential_disintegrations}.
For the necessary mathematical background, as well as the proof of the theorems, we refer the reader to \cref{sec:math_and_proofs}.








\subsection{Gaussian Processes and Gaussian Measure: Background and Equivalence}\label{sec:process_measure_equivalence}
When working with Gaussian priors over function spaces, two complementary
approaches are often used:
~\\
\begin{itemize}
    \item One can work with a  Gaussian process, which is defined as a
        stochastic process  $Z$  over  $D$, such that for 
        any number of points  $x_1, ..., x_n \in D$, the distribution of
         $\left(Z_{x_1}, ..., Z_{x_n}\right)$  is Gaussian, e.g., \citep{tarantola,Sarkka_gp_operator}.
    \item One can work with a
         Gaussian measure  which is defined as a Borel measure on  $C(D)$ 
        such that for any continuous linear functional  $\ell \in C(D)^*$,
        the measure  $\mu \circ \ell^{-1}$ on $\mathbb{R}$  is Gaussian, e.g., \citep{stuart_2010,stuart_dashti,Sullivan2015,Ernst2014}.
\end{itemize}
~\\
For a Gaussian process $Z$ on some set $D$, its mean and covariance function are defined as
\begin{align*}
      m_x &:= \mathbb{E}\left[Z_x\right]\\
        k(x, y) &:= \mathbb{E}\left[Z_x Z_y\right] - \mathbb{E}\left[Z_x\right]\mathbb{E}\left[Z_y\right],
\end{align*}
for any $x, y \in D$. When working with a Gaussian measure $\mu$ over a separable Banach space $X$, these notions are replaced by the \textbf{mean element} and \textbf{covariance operator.}
~\\
\begin{definition}
Given a Gaussian measure $\mu$ on a Banach space $X$, the \textbf{mean} of $\mu$ is the unique element $m_{\mu}\in X$ such that:
\begin{equation}\label{eq:def_mean_element}
    \int_X \langle f, g^*\rangle d\mu(f) = \langle m_{\mu} g^*\rangle,~\forall g^*\in X^*.
\end{equation}
The \textbf{covariance operator} of $\mu$ is the linear operator $C_{\mu}:X^*\rightarrow X$ defined by
\begin{equation}\label{eq:def_covariance_operator}
    C_{\mu}g^* = \int_X \langle f, g^* \rangle f d\mu(f) - \langle m_{\mu}, g^*\rangle m_{\mu},
\end{equation}
where the integrals are to be seen as Bochner integrals. We refer the reader to \citet{Vakhania1987} for more details.
\end{definition}
~\\
When one works over the Banach space of continuous functions $C(D)$ over some compact Euclidean domain $D\subset \mathbb{R}^d$, the Gaussian process and Gaussian measure point of view are equivalent. Indeed, for any Gaussian measure on $C(D)$ there is a corresponding Gaussian process on $D$ with continuous trajectories, and vice-versa (we refer the reader to \cref{sec:equiv_process_measure} for more details about this correspondence). Under this correspondance, the mean and covariance functions of the process may be obtained as special cases of the mean element and covariance operator of the corresponding measure by acting on them with Dirac delta functionals, as shown in the following lemma.
~\\
\begin{lemma}\label{th:corresp_mean_cov}
    Let $Z$ be a Gaussian process on a compact Euclidean domain $D$ with continuous trajectories, and let $\mu$ be the corresponding induced measure on $C(D)$. Then the covariance operator $C_{\mu}$ and mean element $m_{\mu}$ of the measure are related to the mean $m_x$ and covariance function $k(x, y)$ of the process via
    \begin{align}
        m_x &= \mathbb{E}\left[Z_x\right] = \langle m_{\mu}, \delta_x\rangle\label{eq:corresp_mean},\\
        k(x, y) &= \mathbb{E}\left[Z_x Z_y\right] - \mathbb{E}\left[Z_x\right]\mathbb{E}\left[Z_y\right] = \langle C_{\mu}\delta_y, \delta_x \rangle\label{eq:corresp_cov},
    \end{align}
    for all $x, y \in D$.
\end{lemma}
~\\
These considerations allow us to work interchangeably with the two points of views. In the following, we will use the Gaussian measure theory to provide a framework for computing the posterior in linear Bayesian inverse problems under linear form observations.

\begin{remark}
	The correspondance between Gaussian processes and Gaussian measures is not limited to the Banach space $C(D)$ of continuous functions over a compat Euclidean domain. Indeed \citet{rajput_gp_vs_measures} also prove correspondance for $L^p$ spaces and spaces of absolutely continuous functions. However, the proofs are done on a case by case basis, so we choose to restrict ourselves to one single type of Banach spaces.
\end{remark}









\subsection{Disintegration of Gaussian Measures under Operator Observations}\label{sec:disintegration}
Now that we have introduced the equivalence of the process and the measure approaches, we consider the posterior in the Gaussian measure formulation of Bayesian inverse problems. In this setting, conditional laws are defined using the language of \textit{disintegrations} of measures.
The treatment presented here will follow that in \citet{TARIELADZE2007851} and extend some of the theorems therein.\\
~\\
As in \cref{sec:process_measure_equivalence}, we work on the separable Banach space $C(D)$ of continuous functions over a compact Euclidean domain and use $\mu$ to denote a Gaussian measure on $C(D)$ and $Z$ for the corresponding associated Gaussian process on $D$. Again $G:C(D)\rightarrow \mathbb{R}^{\datdim}$ will denote a bounded linear operator. One way to address the conditional law of the measure under observation of $G$ is the concept of \textbf{disintegration}.\\
\begin{definition}\label{def:disintegration}
Given measurable spaces $\left(X, \mathcal{A}\right)$ and $\left(Y, \mathcal{F}\right)$, a probability measure $\mu$ on $X$ and a measurable mapping $G:X\rightarrow Y$, a \textbf{disintegration} of $\mu$ with respect to $G$ is a mapping $\tilde{\mu}:\mathcal{A}\times Y \rightarrow \left[0, 1\right]$ satisfying the properties:
\begin{enumerate}
    \item For each $y \in Y$ the set function $\tilde{\mu}(\cdot, y)$ is a probability measure on $X$ and for each $A \in \mathcal{A}$ the function $\tilde{\mu}(A, \cdot)$ is $\mathcal{F}$-measurable.
    \item There exists $Y_0 \in \mathcal{F}$ with $\mu\circ G^{-1}\left(Y_0\right)=1$ such that for all $y\in Y_0$ we have $\lbrace y \rbrace \in \mathcal{F}$ and for each $y\in Y_0$, the probability measure $\tilde{\mu}(\cdot, y)$ is concentrated on the fiber $G^{-1}\left(\left\lbrace y \right\rbrace\right)$ that is:
    \[
    \tilde{\mu}\left(G^{-1}\left(\left\lbrace y \right\rbrace\right), y\right) = 1.
    \]
    \item The measure $\mu$ may be written as a mixture:
    \[
    \mu\left(A\right) = \int_Y \tilde{\mu}\left(A, y\right)d\left(\mu\circ G^{-1}\right)\left(y\right),~\forall A \in \mathcal{A}.
    \]
\end{enumerate}
We will use the notation $\mu_{|G=y}\left(\boldsymbol{\cdot}\right):=\tilde{\mu}\left(\boldsymbol{\cdot}, y\right)$ for the \textit{disintegrating measure}.
\end{definition}
~\\
In a Bayesian inverse problem, the computation of the posterior then amounts to computing a disintegration of the prior with respect to the observation operator.
The existence of the disintegration is guaranteed by Theorem 3.11 in \citet{TARIELADZE2007851}, which we reproduce here in a slightly adapted formulation generalized to non-centered measures.
~\\
\begin{theorem}\label{th:tarieladze_disintegration}
    Let $X$, $Y$ be real separable Banach spaces and $\mu$ be a Gaussian measure on the Borel $\sigma$-algebra $\mathcal{B}\left(X\right)$ with mean element $m_{\mu}\in X$ and covariance operator $C_{\mu}:X^*\rightarrow X$. Let also $G:X\rightarrow Y$ be a bounded linear operator. Then, provided that the operator $C_{\nu} := GC_{\mu}G^*:Y^*\rightarrow Y$ has finite rank $\datdim$,
    there exists a continuous linear map $\tilde{m}_{\mu}:Y\rightarrow X$, a symmetric positive operator $\tilde{C}_{\mu}:X^*\rightarrow X$ and a disintegration $\left(\mu_{|G=y}\right)_{y\in Y}$ of $\mu$ with respect to $G$ such that for each $y\in Y$ the measure $\mu_{|G=y}$ is Gaussian with mean element $\tilde{m}_{\mu}(y)$ and covariance operator $\tilde{C}_{\mu}$. Furthermore, 
    for any $C_{\nu}$-representing sequence $y_i^*,~i=1, ..., n$, 
    the mean and covariance are equal to
    \begin{align}
        \tilde{m}_{\mu}(y) &= m_{\mu} + \sum_{i=1}^{\datdim} \left\langle y - Gm_{\mu}, y_i^* \right\rangle C_{\mu} G^* y_i^*\label{eq:post_mean_disintegration}\\
        \tilde{C}_{\mu} &= C_{\mu} - \sum_{i=1}^{\datdim} \left\langle C_{\mu}G^* y_i^*, \boldsymbol{\cdot} \right\rangle C_{\mu} G^* y_i^*\label{eq:post_cov_disintegration}.
    \end{align}
    The mean element also satisfies $G\tilde{m}_{\mu}(y) =y$ for all $y\in Y$.
\end{theorem}
~\\
The explicit formulae for the posterior mean and covariance provided by the above theorem require the use of \textbf{representing sequences}.
\begin{definition}{\cite{TARIELADZE2007851}}
Given a Banach space $X$ and a non-zero, symmetric positive operator $R:X^*\rightarrow X$, a family $(x_i^*)_{i\in I}$ of elements of $X^*$ is called $R$-representing if the following two conditions hold:
\begin{align*}
    \langle R x_i^*, x_j^* \rangle &= \delta_{ij},\\
    \sum_{i\in I} \langle R x_i^*, x^*\rangle^2 &= \langle R x^*, x^*\rangle,~\forall x^* \in X^*.
\end{align*}
\end{definition}
\begin{remark}\label{th:remark_rep_seq}
When the operator $R$ has finite rank $\datdim$ and $X$ is an Hilbert space, one can explicitly compute an $R$-representing sequence by defining 
$x_i^*:=R^{-1/2}e_i,~i=1, ..., \datdim$ where $e_i,~i=1,...,\datdim$ is an orthonormal basis of the range of $R$ (see \cref{sec:math_and_proofs} for a proof). This fact will be used to link the posterior provided by \cref{th:tarieladze_disintegration} to the usual formulae for Gaussian processes.
\end{remark}
~\\
Using \cref{th:corresp_mean_cov} we can translate the disintegration provided by \cref{th:tarieladze_disintegration} to the language of Gaussian processes in the case where $X$ is the Banach space $C(D)$ of continuous functions over a compact Euclidean domain $D$:
~\\
\begin{corollary}\label{th:disintegration_gp}
Let $Z$ be a Gaussian process on a compact Euclidean domain $D$ with continuous trajectories and let $G:C(D)\rightarrow Y$ be a linear bounded operator into a real separable Banach space $Y$. Denote by $C_{\mu}$ the covariance operator of the measure associated to the process. Provided the operator $C_{\nu}:= GC_{\mu}G^*$ has finite rank $\datdim$, then, for all $y \in Y$ the conditional law of $Z$ given $G=y$ is Gaussian with mean and covariance function given by, for all $x,x_1,x_2\in D$:
\begin{align*}
    \tilde{m}_x(y) &= \langle \tilde{m}_{\mu}(y), \delta_x \rangle 
    = m_x + \sum_{i=1}^{\datdim} \langle y - G m_{\boldsymbol{\cdot}},
    y^*_i \rangle (C_{\mu}G^*y^*_i)|_x,\\
    \tilde{k}(x_1, x_2) &= \langle \tilde{C}_{\mu} \delta_{x_2}, \delta_{x_1},  \rangle = k(x_1, x_2) -
    \sum_{i=1}^{\datdim} (C_{\mu}G^*y^*_i)|_{x_2} ~ (C_{\mu} G^*y^*_i)|_{x_1},
\end{align*}
where $m_x$ denotes the mean function of $Z$ and $Gm_{\boldsymbol{\cdot}}$ denotes application of the operator $G$ to the mean function seen as an element of $C(D)$ and $\left(y_i^*\right)_{\i=1, ...,\datdim}$ is any $C_{\nu}$-representing sequence.
\end{corollary}
~\\
When $G$ maps into a finite-dimensional Euclidean space, then one can explicitly compute representing sequences and duality pairings, allowing the conditional mean and covariance in \cref{th:disintegration_gp} to be entirely written in terms of the prior mean and covariance function of the process, making the link to the Gaussian process conditioning formulae as found for example in \citet{tarantola}. Indeed, since the dual of $C(D)$ is the space of Radon measures on $D$, any bounded linear operator $G:C(D)\rightarrow \mathbb{R}^{\datdim}$ may be written as a collection of integral operators $GZ = \left(\int_D Z(x) d\lambda_i\left(x\right)\right)_{i=1, ..., \datdim}$ where the $\lambda_i$'s are Radon measures on $D$. This special form allows us to compute closed-from expressions for the conditional mean and covariance.

\begin{corollary}\label{th:link_tarantola}
Consider the situation of \cref{th:disintegration_gp} and let $G:C(D)\rightarrow \mathbb{R}^{\datdim}$ have the form 
$GZ = \left(\int_D Z(x) d\lambda_i\left(x\right)\right)_{i=1, ..., \datdim}$, with the $\lambda_i$'s being Radon measures on $D$.
Then the conditional law of $Z$ given $G=y$ is Gaussian with mean and covariance function given by, for all $x, x_1, x_2\in D$:
\begin{align}
    \tilde{m}_x(y) &= m_x
    - K_{xG}
    K_{GG}^{-1}
    \left(y - Gm_{\boldsymbol{\cdot}}\right)\label{eq:cond_mean_field_fin_dim},\\
    \tilde{k}(x_1, x_2) &= k(x, y) - K_{x_1G} K_{GG}^{-1} K_{x_2G}^T\label{eq:cond_cov_field_fin_dim}
\end{align}
where we have used the compact notation $Gm_{\boldsymbol{\cdot}}$ to denote the application of $G$ to the mean function of the GP seen as an element of $C(D)$ and we have defined the following vectors and matrices:
\begin{align}
    K_{xG} :&= \left(\int_D k(x, y) d\lambda_i\left(y\right)\right)_{i=1,..., \datdim}\in\mathbb{R}^{\datdim}\label{eq:forward_pt_cov_matrix},\\
    K_{GG} :&= \left(\int_D \int_D k(y, z) d\lambda_i\left(y\right) d\lambda_j\left(z\right) \right)_{i,j=1, ..., \datdim} \in \mathbb{R}^{\datdim \times \datdim},\label{eq:forward_cov_matrix}
\end{align}
where $k\left(\boldsymbol{\cdot}, \boldsymbol{\cdot}\right)$ denotes the covariance function of $Z$. 
\end{corollary}

%This makes the final link from the abstract Gaussian measure formulation to the Gaussian process conditioning formulae. Note that in the case of Dirac measure $\lambda=\delta_x$, for some $x \in D$, one recovers the traditional kriging formulae \citep{rasmussen_williams}.













\subsection{Sequential Disintegrations}\label{sec:sequential_disintegrations}
We now turn to the situation where several stages of conditioning are performed sequentially. Let again $X$ be a real separable Banach space and consider two bounded linear operators $G_1:X\rightarrow Y_1$ and $G_2: X \rightarrow Y_2$, where $Y_1$ and $Y_2$ are also real separable Banach spaces. Then, if one views these operators as defining two stages of observations, there is two ways in which one can compute the posterior.
~\\
\begin{itemize}
    \item On the one hand, one can compute it in two steps by first computing the disintegration of $\mu$ under $G_1$ and then, for each $y_1\in Y_1$, compute the disintegration of $\mu_{|G_1=y_1}$ under $G_2$. 
    \item On the other hand, one can compute it in one go by considering the disintegration of $\mu$ with respect to the \textit{bundled} operator $G:X\rightarrow Y_1 \bigoplus Y_2,~x\mapsto G_1\left(x\right) \bigoplus G_2\left(x\right)$. From now one, we will denote this operator by $\left(G_1, G_2\right)$.
\end{itemize}
~\\
We show that these two approaches yield the same disintegration, as guaranteed by the following theorem.
~\\
\begin{theorem}\label{th:transitivity_disintegration}
    Let $X, Y_1,Y_2$ be real separable Banach spaces, $\mu$ be a Gaussian measure on
    $\mathcal{B}\left(X\right)$ with mean element $m_{\mu}$ and covariance
    operator $C_{\mu}:X^*\rightarrow X$. Also let $G_1:X\rightarrow
    Y_1$
    and $G_2:X\rightarrow Y_2$ be bounded linear operators.
    Suppose that both $C_{\nu_1}:= G_1 C_{\mu} G_1^*$ and $C_{\nu_2} :=
    G_2 C_{\mu} G_2^*$ have finite rank $\datdim_1$ and $\datdim_2$, respectively.
    Then
    \[  
        \mu_{|\left(G_1, G_2\right) = \left(y_1, y_2\right)}
        = \left(\mu_{|G_1=y_1}\right)_{|G_2=y_2},
    \]
    where the equality holds for almost all $(y_1, y_2)\in
    Y_1 \bigoplus Y_2$
    with respect to the pushforward measure $\mu\circ \left(G_1,
    G_2\right)^{-1}$ on $Y_1 \bigoplus Y_2$.
\end{theorem}
~\\
Now, since both disintegrating measures are equal, it also follows that all their moments are equal. In the case of finite dimensional data, this yields, using \cref{th:link_tarantola}:
~\\
\begin{corollary}\label{th:update_gp}
Let $Z$ be a Gaussian process on a compact Euclidean domain $D$ with continuous trajectories. Consider two observation operators $G_1:C(D)\rightarrow \mathbb{R}^{\datdim_1},~\left(G_1 Z\right)_i = \int_D Z_x d\lambda_i^{(1)}$ and $G_2:C(D)\rightarrow \mathbb{R}^{\datdim_2},~\left(G_2 Z\right)_i = \int_D Z_x d\lambda_i^{(2)}$. Denote by $m_{\boldsymbol{\cdot}}$ and $k\left(\boldsymbol{\cdot}, \boldsymbol{\cdot}\right)$ the mean and covariance function of $Z$. Then, for any $y = \left(y_1, y_2\right) \in \mathbb{R}^{\datdim_1 + \datdim_2}$ and any $x, x_1, x_2\ in D$, we have:
\begin{align*}
    m_{x} + 
    K_{xG}K_{GG}^{-1}\left(y - Gm_{\boldsymbol{\cdot}}\right)
    &=
    m_{x} + 
    K_{xG_1}K_{G_1G_1}^{-1}\left(y_1 - G_1m_{\boldsymbol{\cdot}}\right)
    + K_{xG_2}\left(\tilde{K}^{(1)}_{G_2G_2}\right)^{-1}\left(y_2 - G_2\tilde{m}^{(1)}_{\boldsymbol{\cdot}}\right),\\
    k(x_1, x_2) - K_{xG}K_{GG}^{-1}K_{yG}^T
    &=
    k(x_1, x_2) 
    - K_{xG_1}K_{G_1G_1}^{-1}K_{yG_1}^T
    - \tilde{K}^{(1)}_{xG_2}\left(\tilde{K}^{(1)}_{G_2G_2}\right)^{-1}\left(\tilde{K}^{(1)}_{yG_2}\right)^T,
\end{align*}
where $G:=\left(G_1, G_2\right)$ and $\tilde{m}^{(1)}$ denotes the conditional mean $Z$ given $G_1=y_1$ as given by \cref{th:link_tarantola}. Also 
$\tilde{K}^{(1)}_{G_2G_2}$ and $\tilde{K}^{(1)}_{xG_2}$ denote the same matrices as in \cref{eq:forward_pt_cov_matrix,eq:forward_cov_matrix} with the prior covariance $k\left(\boldsymbol{\cdot}, \boldsymbol{\cdot}\right)$ replaced by the conditional covariance of $Z$ given $G_1 = y_1$.
\end{corollary}

